On Fairness and Calibration

The machine learning community has become increasingly concerned with the potential for bias and discrimination in predictive models. This has motivated a growing line of work on what it means for a classification procedure to be "fair." In this paper, we investigate the tension between minimizing error disparity across different population groups while maintaining calibrated probability estimates. We show that calibration is compatible only with a single error constraint (i.e. equal false-negatives rates across groups), and show that any algorithm that satisfies this relaxation is no better than randomizing a percentage of predictions for an existing classifier. These unsettling findings, which extend and generalize existing results, are empirically confirmed on several datasets.

==> backup.tex <==
\item Problem setting:
  \begin{itemize}
    \item Given a set of instances $Z$, for each instance $\z = (\x, g, y)$ in $Z$, it has a k-dimensional feature vector $\x \in \R^k$, a group assignment $g$ in the group space $G$, and a label $y$ in the label space $Y$.
    % In the binary classification case, the label space $Y = \{0, 1\}$, while in regression case, the label space $Y = \mathbb{R}$.
    \item Binary Classification:
        \begin{itemize}
            \item The label space $Y$ is $\{-1, +1\}$.
            \item We want to find a fair classifier $\eta \in \mathbb{R}^k \rightarrow [0, 1]$ such that it takes a feature $\x \in \R^k$ and outputs a score $v = \eta(\x)$ that models the conditional probability $\Pr(y_i = +1 | \x)$, i.e. the confidence score of an instance with feature vector $\x$ to have a positive label $y = +1$, while preserving two out of the three fair conditions presented in \cite{kleinberg2016inherent} as follows.
            \item Condition (A) Calibration within the group: for each group $t$ and each score $v$, the probability of a instance in group $t$ with score $v$ which has label $1$ should be equal to $v$ fraction of the probability of a instance in group $t$ with score $v$. In other words, $ \forall t \in G, v \in [0, 1],$
            \begin{align*}
                \Pr_{(\x, g, y) \in Z}(g = t, \eta(\x) = v, y = +1) \\
                = v \cdot \Pr_{(\x, g, y) \in Z}(g = t, \eta(\x) = v)
            \end{align*}
            \item Condition (B) Balance for negative class: the average score of the instances with label $-1$ should be the same across groups. That is, $\forall s, t \in G,$
            \begin{align*}
                \int_{0}^{1} v \Pr_{(\x, g, y) \in Z}(\eta(\x) = v| g = s, y = -1) dv \\
                = \int_{0}^{1} v \Pr_{(\x, g, y) \in Z}(\eta(\x) = v| g = t, y = -1) dv
            \end{align*}
            \item Condition (C) Balance for positive class: the average score of the instances with label $+1$ should be the same across groups. That is, $\forall s, t \in G,$
            \begin{align*}
                \int_{0}^{1} v \Pr_{(\x, g, y) \in Z}(\eta(\x) = v| g = s, y = +1) dv \\
                = \int_{0}^{1} v \Pr_{(\x, g, y) \in Z}(\eta(\x) = v| g = t, y = +1) dv
            \end{align*}
        \end{itemize}
    \item 
  \end{itemize}

==> sections/feasibility.tex <==
%!TEX root=../main.tex
\section{Feasibility}
\label{sec:feasibility}

We now show Calibration-Preserving Parity is a feasible definition
of fairness through a proof by construction. We will show that it is possible
derive calibrated classifiers with minimal disparity from classifiers that do
not meet this condition.

Assume we are given classifiers $h_1$ and $h_2$ for groups $G_1$ and $G_2$.
$h_1$ and $h_2$ do not achieve the disparity condition, but are approximately
calibrated --- i.e.  both $\calib{h_1}$ and $\calib{h_2}$ are small.\footnote{
  If this is not the case, one could improve calibration
  with Platt Scaling \cite{platt1999probabilistic} or
  isotonic regression \cite{zadrozny2001obtaining}.
}
Without loss of generality, for the remainder of the paper we assume that
\fairconst{h_1}{1} is larger than \fairconst{h_2}{2}.
We will show that, under minor assumptions, that is is possible to achieve
Calibration-Preserving Parity with respect to $\fairconstname$:
%
\begin{thm}[Feasibility]
  Let $h_1$ and $h_2$ be defined as above. If $\fairconst{h_1}{1} \leq
  \argmax_{h^*_2 \in \mathcal{H}^*_2} \fairconst{h^*_2}{2}$, where
  $\mathcal{H}^*_2$ is the set of calibrated classifiers for group $G_2$,
  then there exists some classifier $\fair h_2$ for group $G_2$ with
  $\calib{\fair h_2} \leq \calib{h_2}$ and $\fairconst{h_1}{1} = \fairconst{\fair h_2}{2}$.
  \label{thm:feasibility}
\end{thm}

To show that this is possible, we will derive a new classifier $\fair h_2$ that
replaces some predictions of $h_2$ with predictions from a ``trivial
classifier'' $h^\triv_2$ that simply outputs the base rate $\br_2$
on all inputs (i.e. $\forall \x$, $h^\triv_2(\x) = \br_2$).
Specifically, for some Bernoulli variable $B$ with expectation $\alpha$,
%
\begin{equation}
  \fair{h}_2(\x) = (1 - B) h_2(\x) + B h^\triv_2(\x).
  \label{eqn:fair_classifier}
\end{equation}
%
Intuitively, by modifying the parameter $\alpha$, we are interpolating between the two classifiers
$h_2$ and $h^\triv_2$, and thus interpolating between their costs.
A geometric interpretation of this can be seen in \autoref{fig:postprocess}.
By modifying the replacement rate $\alpha$, we can raise and lower the cost of $\fair h_2$.
Setting
$ \alpha = \frac{\fairconst{h_1}{1} - \fairconst{h_2}{2}}{\fairconst{h^\triv_2}{2} - \fairconst{h_2}{2}}$
ensures that the cost of $\fair h_2$ matches that of $h_1$ (see \autoref{thm:interpolation}
in \autoref{sec:detailed-feasibility}).
Moreover, the resulting $\fair h_2$ will be at least as calibrated as $h_2$
(see \autoref{thm:calibration} in \autoref{sec:detailed-feasibility}).
Therefore, $h_1$ and $\fair h_2$ will satisfied
Calibration-Preserving Parity with respect to \fairconstname.
We summarize these steps in \autoref{alg:method}, and prove that it meets the
conditions of \autoref{def:fair} in the supplementary material.
%
\begin{algorithm}
  \caption{\methodname{} by post-processing}
  \label{alg:method}
  \begin{algorithmic}
    \STATE {\bfseries Input:} classifiers $h_1$ and $h_2$ s.t.
    $\fairconst{h_2}{2} \leq \fairconst{h_1}{1} \leq \fairconst{h^\triv_2}{2}$, holdout set $P_{valid}$

    \begin{itemize}
      \STATE Determine base rate $\br_2$ of $G_2$ (using
        $P_{valid}$) to produce trivial classifier $h^\triv_2$

      \STATE Construct $\fair h_2$ using \eqref{eqn:fair_classifier} with
        $ \alpha = \frac{\fairconst{h_1}{1} - \fairconst{h_2}{2}}{\fairconst{h^\triv_2}{2} - \fairconst{h_2}{2}}$,
        where $\alpha$ is the interpolation parameter.
    \end{itemize}

    \RETURN $h_1$, $\fair h_2$.
  \end{algorithmic}
\end{algorithm}

\paragraph{Limitations.}
%
It is worth noting the cases in which \methodname{} is infeasible. For the following cases,
we assume that we cannot improve the cost $h_1$ and $h_2$ with further training
or postprocessing, given a finite set
of data and features.\footnote{
  Otherwise, the improved classifier would then be the input to \autoref{alg:method}.
}
%
\begin{corollary}
  \methodname{} is infeasible if
  $\fairconst{h_1}{1} > \argmax_{h^*_2 \in \mathcal{H}^*_2} \fairconst{h^*_2}{2}$.
  %where $\mathcal{H}^*_2$ is the set of all calibrated classifiers for group $G_2$.
  \label{crly:infeasible_trivial}
\end{corollary}
%
\begin{corollary}
  \methodname{} is infeasible if group membership $G_t$ is more predictive
  than any features --- i.e., if
  $ \fairconst{h^\triv_t}{t} \leq \fairconst{h'_t}{t}$, where $h'_t$ is
  any (possibly uncalibrated) classifier.
  \label{crly:infeasible_predictive}
\end{corollary}
%
\begin{corollary}
  In all other cases, \autoref{alg:method} will achieve \methodname{}.
  \label{crly:method_works}
\end{corollary}
%
(Recall that $\mathcal{H}^*_t$ is the set of calibrated classifiers for group $G_t$.)
\autoref{crly:infeasible_trivial} is trivially true because we cannot find a
calibrated classifier for group $G_2$ with cost equal to $\fairconst{h_1}{1}$.
\autoref{crly:infeasible_predictive} is a direct consequence of this result, combined with the fact that
the trivial classifier $h^\triv_t$ is the calibrated classifier for group $G_t$ that
maximizes any cost function of the form \eqref{eqn:cost_general}
(see \autoref{lma:trivial} in \autoref{sec:detailed-feasibility}).
To see why \autoref{crly:method_works} holds, note that \autoref{alg:method}
can match the cost of any classifier in the range $\left[ \fairconst{h_2}{2}, \fairconst{h^\triv_2}{2} \right]$
(see \autoref{thm:interpolation}).
Because $h^\triv_2$ maximizes cost, \autoref{alg:method} will fail only if
$\fairconst{h_1}{1} \geq \fairconst{h^\triv_2}{2} = \argmax_{h^*_2 \in
\mathcal{H}^*_2} \fairconst{h^*_2}{2}$, in which case \methodname{} is
infeasible.

%\paragraph{Relation to Equalized Odds via post-processing}

%\autoref{alg:method} provides an interesting connection to the work of
%\citet{hardt2016equality}, who
%provide a post-processing method to achieve Equalized Odds (false-positive
%and false-negative constraints without calibration).
%Their method amounts to a linear program over two dimensions, which is exactly
%what one would expect given that they are optimizing over a four-dimensional
%space with two linear constraints, leaving two free variables to optimize over.
%\autoref{alg:method} is a linear program over one dimension, as calibration
%constraints the set of classifiers to a one-dimensional space.
%\gp{This maybe goes to supplementary\ldots}




==> sections/introduction_.tex <==
%!TEX root=../main.tex
\section{Introduction}
Machine learning is being used increasingly to assess risk in various domains,
including the criminal justice system, online advertising, and
medical testing \cite{whitehouse-big-data}.
%Fundamentally, a tool for assessing risk can be viewed as assigning
%each individual an estimate of the probability that they belong
%to the positive class in a classification problem.
As with any application of machine learning, these risk assessments
will be carried out with some underlying level of error.
Recently, there has been growing concern
that these errors are made in ways that systematically discriminate against
particular groups of people \cite{barocas2016big,berk2017fairness,chouldechova2017fair}.
%
% Example time
% \kilian{ I am not sure about this example, not everybody may agree.}
A recent high-profile example of these concerns was raised by the
news organization ProPublica, who studied a risk tool
that is widely used in the criminal justice system.
This tool assigns to each criminal defendant an estimated probability
that they will commit a future crime.
ProPublica found that the risk estimates assigned to
defendants who didn't go in to commit future crimes were on average
higher among African-American defendants than Caucasian defendants \cite{angwin-propublica-risk-scores}.
Assigning non-trivial risk to people who didn't in fact commit a
crime in the future is a form of false-positive error, and in this case it
disproportionately affected African-American defendants.

To mitigate issues such as these,
the machine learning community has proposed different
frameworks which attempt to quantify fairness in classification
\cite{barocas2016big,berk2017fairness,chouldechova2017fair,hardt2016equality,kleinberg2016inherent,woodworth2017learning,zafar2017fairness}.
A recent and particularly noteworthy framework is Equalized Odds \cite{hardt2016equality}
(also referred to as Disparate Mistreatment \cite{zafar2017fairness}),
which constrains classification algorithms such that no error type (false-positive
or false-negative) disproportionately affects any population subgroup.
This notion of non-discrimination is feasible in many settings,
and researchers have developed tractable algorithms for achieving it \cite{hardt2016equality,goh2016satisfying,zafar2017fairness,woodworth2017learning}.
%
%These include trying to ensure \emph{individual fairness}
%\cite{dwork2012fairness}; training classifiers to
%guarantee fairness with respect to \emph{groups}, where a group may refer to a
%particular race, gender, or other subset of the population
%\cite{calders2009building,kamiran2009classifying,calders2010three}; and obfuscating the
%feature representation of individuals to remove any information of group
%membership \cite{zemel2013learning, louizos2015variational,
%edwards2015censoring}.

\noindent\textbf{Calibration.}
However, equalized error rates do not necessarily remove all potential
for discrimination.
When risk tools are used in practice, a key goal is that they be
{\em calibrated}: if we look at the set of people who receive a probability
of $p$, we would like a $p$ fraction of the members of this set to
in fact be positive instances of the classification
problem \cite{dawid1982well}.
Moreover, if we are concerned about fairness between two groups
$G_1$ and $G_2$ (e.g. African-American defendants and white defendants)
then we would like this calibration condition
to hold simultaneously for the set
of people within each of these groups as well
%: of all people in group $G_t$
%who are labeled $p$ (for $t = 1, 2$), a $p$ fraction should be
%positive instances
\cite{flores-re-propublica-fair}.
%
% Calibration is in a sense a necessary condition for a risk tool if it
% is going to be used as intended in practice.
Calibration is a crucial condition for a risk tool in many settings.
If a risk tool for
evaluating defendants were not calibrated with respect to groups
defined by race, for example, then a probability estimate of $x$
could mean different things for African-American and white defendants,
and hence the tool would have the unintended, and highly undesirable,
consequence of incentivizing judges to take race into account when
interpreting its predictions.\footnote{There are many similar examples.
Suppose a tool for estimating the probability that a medical student
will succeed as a doctor were uncalibrated with respect to gender,
and suppose this tool were used to inform hospital hiring decisions.
Then it could become rational for patients choosing a doctor to take the
doctor's gender into consideration as a criterion in their choice.}

Despite the importance of calibration as a property,
our understanding of how it interacts
with other fairness properties is limited.
We do know from recent work that,
except in the most constrained
cases, it is impossible to achieve calibration while also
satisfying the Equalized Odds framework
\citep{kleinberg2016inherent,chouldechova2017fair}.
However, we do not know how best to achieve relaxations of these guarantees
that might be feasible in practice, or how calibration may be
combined with other definitions of fairness.

\noindent\textbf{Our Contributions.}
In this paper, our goal is to further investigate the relationship
between calibration and equalized error rates.
Our results generalize the work of \citet{kleinberg2016inherent}
and \citet{chouldechova2017fair}, who first observed the incompatibility
between calibration and Equalized Odds.
We characterize the set of calibrated classifiers for different population
groups with a surprisingly simple geometric intuition.
From this intuition, we can derive a number of straightforward
yet profound implications.
%
Firstly, while there are notions of error-rate non-discrimination that are compatible
with calibration, we show that such instances require a significant
relaxation of the equalized odds conditions.
Additionally, any such notions become infeasible when the prediction task
is inherently noisy, or when population group membership is a strong predictive
feature.
Finally, we demonstrate that achieving calibration and even the most simple
non-discrimination constraints inherently incurs a non-trivial performance
cost, which may be inadvisable in many situations.
In the supplementary material, we show that all of these findings hold in
an approximate sense as well; the (in)feasibility and performance
costs degrade smoothly as the calibration condition is relaxed.
We demonstrate these findings both theoretically and empirically,
comparing calibrated notions of non-discrimination against
the (uncalibrated) Equalized Odds framework on several datasets.
Our conclusion is that calibration and error-rate constraints are in
most cases mutually incompatible goals, and therefore practitioners
should choose only one of these goals rather than attempting to achieve
some relaxed notion of both.

\gp{
There is a unique solution
can be achieved by a simple interpolation algorithm
is unadvisable in many situations.
}

\gp{
Can't do better than a random coin toss.
}

\gp{
There has been a cry for fairness.
}

\gp{
Here's a natural way of thinking about fairness.
This simple geometric intuition makes it crystal clear
that this notion is simply achievable, but unsatisfying because of coin toss.
}

\gp{
Get rid of \methodname{}.
}


==> sections/optimality.tex <==
\section{Optimality}
\label{sec:optimality}

\gp{A troublesome optimality result}

\gp{Uniqueness + implications}

\gp{Can't do better than a random coin toss.}

In this section, we prove that the post-processing method \autoref{alg:method}
produces a solution which is not only feasible but also near-optimal over
\emph{all} non-discriminatory classifiers with respect to generalized
false-positive and false-negative rates. Intuitively, this holds because,
under the calibration constraint, the cost of a classifier uniquely determines
the false-positive/false-negative rates for a given base rate $\mu_t$:
%
\begin{lemma}
  Let $h_t$ and $h'_t$ be perfectly calibrated classifiers with cost
  $\fairconst{h_t}{t} \leq \fairconst{h'_t}{t}$ for some
  cost function $\fairconstname$. Then $\fp{h_t} \leq \fp{h'_t}$
  and $\fn{h_t} \leq \fn{h'_t}$, with equality only if $\fairconst{h_t}{t} = \fairconst{h'_t}{t}$.
  \label{lem:fpfn_exact}
\end{lemma}
%
This also holds in an approximate sense if $h_t$ and $h'_t$ are approximately
calibrated (see \autoref{lem:fpfn} in \autoref{sec:cost_and_error}).
As described in \autoref{sec:setup}, the false-positive rate of a calibrated classifier
determines the false-negative rate, and vice versa. Because cost functions
of the form given by \eqref{eqn:cost_general} are positive combinations of
the false-positive/false-negative rates, it can be seen that there is only one
false-positive/false-negative solution for a given cost value, and improving one
of the values strictly improves the others.
The geometric intuition of this can be seen in \autoref{fig:postprocess}:
the level-order curves of $\fairconstname$ intersect the set of
calibrated classifiers in one point on the false-positive/false-negative plane.

Our goal is to find classifiers that simultaneously minimize the
false-positive/false-negative costs for both groups $G_1$ and $G_2$, subject to a
calibration constraint and non-disparity.
We continue with the assumption that, given a finite set of data and features,
we cannot strictly improve the cost (and therefore the
false-positive/false-negative rates) of the discriminatory classifiers $h_1$ and $h_2$.
Therefore, non-discriminatory classifiers with cost lower than that of
$\fairconst{h_1}{1}$ are infeasible (again assuming without loss of
generality that $\fairconst{h_1}{1} \geq \fairconst{h_2}{2}$).
Note that \autoref{alg:method} produces a classifier $\fair h_2$ with cost equal
to $\fairconst{h_1}{1}$, therefore achieving the minimum possible
cost for non-discriminatory classifiers. If we assume that $h_1$ and $\fair h_2$
are perfectly calibrated, then by \autoref{lem:fpfn_exact} $h_1$ and $\fair h_2$
must also achieve the minimum possible false-positive and false-negative rates
for non-discriminatory classifiers, and thus are optimal. This is summarized below:
%
\begin{thm}[Optimality of \autoref{alg:method}]
  Let $h_1$ and $h_2$ be (discriminatory) classifiers which achieve the
  minimum false-positive and false-negative rates for groups $G_1$ and $G_2$, respectively
  (i.e. cannot be strictly improved).
  If $h_1$ and $h_2$ are perfectly calibrated, then \autoref{alg:method} produces
  the optimal perfectly calibrated non-discriminatory classifiers with respect
  to false-positive/false-negative rates.
  \label{thm:optimality}
\end{thm}
%
\autoref{thm:optimality} holds in an approximate sense as well:
if $h_1$ and $h_2$ are approximately (but not perfectly) calibrated, then
\autoref{alg:method} produces non-discriminatory classifiers which are
near-optimal among classifiers that are just as calibrated as $h_1$ and $h_2$.
We formalize this in \autoref{thm:approx-fp-optimality} and
\autoref{thm:approx-fn-optimality} in \autoref{sec:optimality-proofs}.

%\paragraph{Bounding Generalized False-Positive and False-Negative Rates.}
%We can show that our postprocessing technique is near-optimal with respect
%to generalized false-positive and false-negative rates.
%We assume that the given classifier $h_1$ is Pareto-dominant in the sense that
%we cannot find a strictly better classifier $h_1'$ that is at least as
%calibrated as $h_1$ but has strictly smaller generalized false-positive or false-negative
%rate. As a consequence, $\fairconst{h_1}{1}$ and $\fairconst{\fair
%h_2}{2}$ must both be at least $\fairconst{h_1}{1}$. (We formalize this with \autoref{lem:fpfn}
%in the supplementary material).
%As a result, assuming that $h_1$ was
%Pareto-dominant, any classifiers satisfying our calibration and disparity
%constraints must have generalized false-positive and false-negative rates
%approximately equal to those of our derived classifiers $h_1$ and $\fair
%h_2$.

\paragraph{Relation to Equalized Odds post-processing.}
It is worth noting that \autoref{thm:optimality} implies that
the classifiers produced by \autoref{alg:method} are optimal not
only for post-processing methods but among \emph{all}
calibrated classifiers.
\gp{How to word this better?}
%
This is in contrast this with the (uncalibrated) Equalized Odds
framework, in which post-processing methods do not always produce
the optimal non-discriminatory classifier.
\citet{woodworth2017learning} show that the post-processing method
of \citet{hardt2016equality} may be suboptimal when group membership
is more predictive than any other feature.
It is worth noting that this result does not directly apply to
\methodname{} non-discrimination.
Firstly, \methodname{} is infeasible when group membership is the
most predictive feature (\autoref{crly:infeasible_predictive}), and
therefore the suboptimality result of \cite{woodworth2017learning} does
not apply.
Moreover, the feasibility region of classifiers for \methodname{}
is sufficiently more restrictive than that of Equalized Odds, which
makes optimization through post-processing tractable.
Equalized Odds solutions may lie anywhere in the false-positive/false-negative
plane, as the framework affords two degrees of freedom. As the post-processing
method of \cite{hardt2016equality} confines solutions to a limited subregion of the
plane it is possible that the derived classifiers may not be optimal. However,
solutions to \methodname{} are restricted to a line in the false-positive/false-negative
plane. As \autoref{alg:method} can derive all possible classifiers in this subspace
(again assuming we cannot strictly improve upon $h_1$ and $h_2$), then a solution
solution which is optimal with respect to the post-processing method \autoref{alg:method}
must be optimal over all (achievable) non-discriminatory solutions.

\paragraph{Implications.}
The optimality of \autoref{alg:method} is beneficial for many reasons.
Beyond ease of implementation, post-processing algorithms offer visibility into
the performance/disparity trade-off, whereas training-time constraints make
this tradeoff harder to see. It is therefore easy for a practitioner to change
the post-processing parameters to select a desirable balance between
performance and non-disparity. \gp{Copied directly from the rebuttal. Does it belong here?}

However, in some applications, the cost of randomizing predictions for the
stronger group ($G_2$) may not be a suitable option. In such cases, the only path towards
non-discrimination is improving the classifier for the weaker group ($G_1$)
either by collecting more data, using additional features, or denoising existing
data. When this extra work is not possible, achieving non-discrimination will
require a sacrifice in performance, as is the case with other frameworks
of fairness
\cite{berk2017fairness,corbett2017algorithmic,hardt2016equality,zliobaite2015relation}.
\gp{Trying to hammer the point home here, but a bit overkill maybe?}
In these settings, \autoref{alg:method} is
the best solution to achieve non-discrimination with calibration.

%such that $\epsilon(h_1') \le
%\epsilon(h_1)$
%and $\fp{h_1'} < \fp{h_1}$ or $\fn{h_1'} < \fn{h_1}$.

